Boosting Neural Machine Translation

Training efficiency is one of the main problems for Neural Machine Translation (NMT). Deep networks need for very large data as well as many training iterations to achieve state-of-the-art performance. This results in very high computation cost, slowing down research and industrialisation. In this paper, we propose to alleviate this problem with several training methods based on data boosting and bootstrap with no modifications to the neural network. It imitates the learning process of humans, which typically spend more time when learning "difficult" concepts than easier ones. We experiment on an English-French translation task showing accuracy improvements of up to 1.63 BLEU while saving 20% of training time.

==> 1M_corpus_table.tex <==
\begin{table}[h!]
\centering
\scriptsize
 \begin{tabular}{llccc}
\hline 
 \textit{Type} & $\#$ \textit{lines}  &  $\#$ \textit{src tok (EN)} & $\#$ \textit{tgt tok (FR)} \\
\hline 
Train & 1M     & 24M & 26M  \\
Valid & 2,000  & 48K & 55K  \\
Test &  2,000 & 48K & 54K    \\
%& nc-2007 & 2,007 & 51K & 62K \\
\hline 
 \end{tabular}
 \caption{\label{tab:XP_DA}Data used to train the model.}
\end{table}

==> 1M_single_no_shuffle.tex <==


\begin{figure}
  \begin{tikzpicture}
    \begin{axis}[
      xlabel={Epoch},
      ylabel={BLEU},
      xmin=1, xmax=18,
      ymin=36, ymax=55,
      %xtick={1,3,5,7,9,11,13,15,17},
      xtick={2,4,6,8,10,12,14,16,18},
      ytick={36,38,40,42,44,46,48,50,52,54},
      width=0.45\textwidth,
      ymajorgrids=true,
      grid style=dashed,
      legend pos=south east,
      legend cell align=left,
      legend style={font=\tiny, draw=none},
      ]
      \addplot[
      color=black,
      mark=triangle,
      ]
      coordinates {
%default
(1, 38.85)
(2, 44.45)
(3, 45.58)
(4, 47.37)
(5, 48.15)
(6, 48.52)
(7, 49.15)
(8, 49.67)
(9, 49.36)
(10, 50.55)
(11, 50.83)
(12, 51.77)
(13, 52.31)
(14, 52.27)
(15, 52.44)
(16, 52.61)
(17, 52.59)
(18, 52.49)
      };
      \addplot[
      color=red,
      mark=square,
      ]
      coordinates {
%no shuffle at all
(1, 35.86)
(2, 34.89)
(3, 38.22)
(4, 40.76)
(5, 41.11)
(6, 43.32)
(7, 42.64)
(8, 43.83)
(9, 44.83)
(10, 47.43)
(11, 50.14)
(12, 51.3)
(13, 51.77)
(14, 52.44)
(15, 52.87)
(16, 53.17)
(17, 53.23)
(18, 53.38)
      };
      \addplot[
      color=blue,
      mark=diamond,
      ]
      coordinates {
%boosting 10%
(1, 35.79)
(2, 45.02)
(3, 47.46)
(4, 49.39)
(5, 50.46)
(6, 50.68)
(7, 50.63)
(8, 51.67)
(9, 52.85)
(10, 53.26)
(11, 53.56)
(12, 53.76)
(13, 53.69)
(14, 53.84)
(15, 53.88)
(16, 53.87)
(17, 54.01)
(18, 53.92)
      };
      \addplot[
      color=green,
      mark=star,
      ]
      coordinates {
%reduction 80% restart every 3 epochs
(1, 35.79)
(2, 40.62)
(3, 43.12)
(4, 47.88)
(5, 46.3)
(6, 49.24)
(7, 51.13)
(8, 51.24)
(9, 51.95)
(10, 52.91)
(11, 52.5)
(12, 52.84)
(13, 53.2)
(14, 53.25)
(15, 53.21)
(16, 53.25)
(17, 53.44)
(18, 53.39)
      };
      \legend{default (shuffle), default (no shuffle), boosting 10\% (no shuffle), reduce 20\% (no shuffle)}
    \end{axis}
  \end{tikzpicture}
  \caption{Effect of data boosting and data reduction with no shuffled orders and training with all 100\% ordered data for each epoch.}
  \label{fig:boosting_bleu_no_shuffle}
\end{figure}


==> 1M_single_table.tex <==
\begin{table}[]
\centering
\footnotesize
\begin{tabular}{l|c|c|c}
\hline
                    & Acc.           & \begin{tabular}[c]{@{}c@{}}Acc.\\(no shuffling)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training\\cost\end{tabular} \\ \hline
baseline (default)  & 52.49          & 53.38                                                       & 100\%         \\ \hline
boosting 10\%       & 53.98          & 53.92                                                       & 110\%         \\ \hline
reduce 20\%         & \textbf{54.12} & 53.39                                                       & \textbf{80\%} \\ \hline
bootstrap 100\%     & 53.36          &                                                             & 100\%         \\ \hline
Ensemble (4 models) & 55.04          &                                                             &               \\ \hline
\end{tabular}
\caption{\label{tab:bleu}BLEU scores (epoch18) and training cost for different systems on a held-out testset (with and without shuffling).}
\end{table}
